Benchmarking Universal Machine Learning Interatomic Potentials on Elemental Systems

The rapid emergence of universal Machine Learning Interatomic Potentials (uMLIPs) has transformed materials modeling. However, a comprehensive understanding of their generalization behavior across configurational space remains an open challenge. In this work, we introduce a benchmarking framework to evaluate both the equilibrium and far-from-equilibrium performance of state-of-the-art uMLIPs, including three MACE-based models, MatterSim, and PET-MAD. Our assessment utilizes Equation-of-State (EOS) tests to evaluate near-equilibrium properties, such as bulk moduli and equilibrium volumes, alongside extensive Minima Hopping (MH) structural searches to probe the global Potential Energy Surface (PES). Here, we assess universality within the fundamental limit of unary (elemental) systems, which serve as a necessary baseline for broader chemical generalization and provide a framework that can be systematically extended to multicomponent materials. We find that while most models exhibit high accuracy in reproducing equilibrium volumes for transition metals, significant performance gaps emerge in alkali and alkaline earth metal groups. Crucially, our MH results reveal a decoupling between search efficiency and structural fidelity, highlighting that smoother learned PESs do not necessarily yield more accurate energetic landscapes.

==> Makefile <==

MAINFILE = main
SI = SI

#TEX = lualatex
TEX = pdflatex

TARGETS = main SI

all: 	pdf

si: 	pdfsi

clean:
	$(foreach i,$(TARGETS),rm -f $i.ps $i.aux $i.dvi $i.log	\
	$i.bbl $i.blg $i.end $iNotes.bib $i.out $i.toc $i.pdf;)

flush:	clean
	$(foreach i,$(TARGETS),rm -f  $i.pdf $i-sm.pdf;)

veryclean: clean
	rm -v -f $(FIGS)

quik:
	$(TEX) $(MAINFILE).tex

#cleanall: clean
#	$(MAKE) -C data clean
#
.FORCE:
diff: .FORCE
	git show HEAD~$(R1):$(MAINFILE).tex >rev$(R1).tex
	git show HEAD~$(R2):$(MAINFILE).tex >rev$(R2).tex
	latexdiff rev$(R1).tex rev$(R2).tex >diff_$(MAINFILE).tex
	pdflatex diff_$(MAINFILE)
	rm -f rev$(R1).tex rev$(R2).tex diff_$(MAINFILE).aux	\
	diff_$(MAINFILE).log diff_$(MAINFILE).out		\
	diff_$(MAINFILE).tex
#   example: make diff R1=1 R2=0 

diff2: .FORCE
	git show HEAD:$(MAINFILE).tex >rev1.tex
	cp $(MAINFILE).tex rev2.tex
	latexdiff rev1.tex rev2.tex >diff_$(MAINFILE).tex
	pdflatex diff_$(MAINFILE)
	rm rev1.tex rev2.tex diff_$(MAINFILE).aux	\
	diff_$(MAINFILE).log diff_$(MAINFILE).out	\
	diff_$(MAINFILE).tex


$(MAINFILE).ps: $(MAINFILE).dvi
	dvips -D 600 $(MAINFILE).dvi

ps: $(MAINFILE).ps


pdf: $(MAINFILE).pdf

pdfsi: $(SI).pdf

$(SI).pdf:	$(SI).tex main.bib
	$(TEX) $(SI).tex
	#bibtex $(SI)
	$(TEX) $(SI).tex
	$(TEX) $(SI).tex
	
$(MAINFILE).pdf: $(MAINFILE).tex $(MAINFILE).bib #$(FIGS) #bigtable.tex
	$(TEX) $(MAINFILE).tex
	bibtex $(MAINFILE)
	$(TEX) $(MAINFILE).tex
	$(TEX) $(MAINFILE).tex
#
#figs/test/FIG1.pdf:
#	epstopdf figs/test/FIG1.eps --outfile=figs/test/FIG1.pdf

small: $(MAINFILE).pdf 
	$(foreach i,$(TARGETS), gs -sDEVICE=pdfwrite			\
	-dCompatibilityLevel=1.4 -dPDFSETTINGS=/prepress -dNOPAUSE	\
	-dQUIET -dBATCH -sOutputFile=$(i)-sm.pdf $(i).pdf;)

